Discourse Coherence, Reference Grounding and Goal Oriented Dialogue

Prior approaches to realizing mixed-initiative human--computer referential communication have adopted information-state or collaborative problem-solving approaches. In this paper, we argue for a new approach, inspired by coherence-based models of discourse such as SDRT \cite{asher-lascarides:2003a}, in which utterances attach to an evolving discourse structure and the associated knowledge graph of speaker commitments serves as an interface to real-world reasoning and conversational strategy. As first steps towards implementing the approach, we describe a simple dialogue system in a referential communication domain that accumulates constraints across discourse, interprets them using a learned probabilistic model, and plans clarification using reinforcement learning.

==> Brian.tex <==
\subsection{Reference Model Description}
\label{composite_model}
For generating and interpreting color patch descriptions, we build and extend the speaker reasoning models of \citet{Brian-Matthew-SigDial} to better capture the flexibility of individual speakers.  
%
First, we extend the \textsc{Referential Goal Composition} (RGC) model, which computes the likelihood that a color description applies to one color patch and not another as differences in linguistic meanings. 
%
The extension leverages previous work on Bayesian Neural Networks \cite{bayesbybackprop} to fit the parameters of a Gaussian prior distribution with a spike-and-slab Gaussian hyper-prior for the weights of the final Linear layer.
%
We name the extended model \textsc{Stochastic Referential Goal Composition} (S-RGC) because it stochastically samples a range of meanings from the learned prior distribution to distinguish between two color patches in potentially different ways. 
%
To fit S-RGC's parameters, we minimize KL-divergence loss that measures the distance from the prior to the hyper-prior in addition to the language model and applicability calibration losses of \citet{Brian-Matthew-SigDial}. 


Next, we ensemble S-RGC, a linguistic reasoning model, with the cooperative reasoning and conservative baseline models to create a composite model. 
%
We follow the methodology of \citet{Brian-Matthew-SigDial}, which first fits the three models' parameters to the XKCD dataset, and then ensembles them on the Colors In Context dataset. 
% 
The ensembling uses a mixture model formulation and an Expectation-Maximization (EM) routine to minimize the perplexity of the training split of the Colors in Context dataset. 
%
The S-RGC and the conservative baseline each have a single tunable hyper parameter that do not control the model size, but the behavior of the model. 
%
We select among them by instantiating 20 possible settings for each, fitting a mixture model for all 400 combinations, and choosing the mixture that has the lowest perplexity on the development split of the Colors in Context dataset.

==> cuts.tex <==
%
%The first step in describing this regression is 
%
%Our Q-function approximator includes a single linear layer that maps a state of $d$ dimensions with $num\_dialogue\_acts = 6$. 

% Since the lengths of the conversations can vary, we defined a parameter $max\_dialogue\_length$ which we set to $15$. 
% %
% Actions are represented using one hot encoding vectors so the dimensions $d$ of each state would be $d=num\_dialogue\_acts=6 * max\_dialogue\_length=15 + 3$. 
% %
% This gives us a vector-based representation of each state \ref{state_ref}. 
%

% which
% could be used by simulations to reason for the next dialogue act and build more and more complex user simulations. Since probabilities are continuous in the interval $[0, 1]$ 
% we use DQNs to implement the RL simulation. 

% Our Q-function approximator consists of a single linear layer which maps a state of $d$ dimensions with $num\_dialogue\_acts = 6$.



==> extra-material.tex <==
\subsection{Available Actions}
\label{ActionSpace}
In our system, we had six actions to choose for both the director (speaker) and matcher (listener). The actions (we will be using bullet labels below in pseudo-code) and their logical forms are as follows:
\begin{enumerate}
    \item \textit{IDENTIFICATION}: Identify the color description using language. It is represented as:\\ 
    IDENTIFY(T, COLOR\_TERM).
    
    \item \textit{ASK\_CLARIFICATION}: Sample a color patch according to the current posterior distribution and ask a clarification question about it. It is represented as:\\ 
    ASK\_CLARIFICATION(T, A) AND IDENTIFY(A, COLOR\_TERM).
    
    \item \textit{CONFIRMATION}: Assertion that the given description is the correct one. It is represented as:\\
    CONFIRMATION(T)\\
    Where T refers to the color patch in the previous iteration.
    
    \item \textit{REJECTION}: This actions asserts that the given description of the color patch is not the correct one and provides with a new description as well. It is represented as:\\
    REJECTION(T, A) AND IDENTIFY(A, COLOR\_TERM)
    
    \item \textit{SELECTION}: This action of chooses the color patch with maximum probability. This action can only be executed by the matcher.\\
    REJECTION(T, A) AND IDENTIFY(A, COLOR\_TERM)
    
    \item \textit{NONE}: This action was for when the director provided with a description which the matcher could not understand.
    
\end{enumerate}


























\begin{figure}[th!]
\centering
\begin{tabular}{l}
    \multicolumn{1}{c}{
        \shortstack{\ColorSquare{semdial4target} \\ $x_0$}
        \shortstack{\ColorSquare{semdial4alt1} \\ $x_1$}
        \shortstack{\ColorSquare{semdial4alt2} \\ $x_2$}
    } \\
    \begin{tabular}{|ll|} 
    \hline
        director: & bright purple \\
        matcher: & reddish or bluish? \\
        director: & true purple \\
 \hline
 \end{tabular}
 \end{tabular}
 \caption{Alternate figure for Matthew}
\end{figure}

\begin{figure}[th!]
\centering
\begin{tabular}{l}
    \multicolumn{1}{c}{
        \shortstack{\ColorSquare{semdial5target} \\ $x_0$}
        \shortstack{\ColorSquare{semdial5alt1} \\ $x_1$}
        \shortstack{\ColorSquare{semdial5alt2} \\ $x_2$}
    } \\
    \begin{tabular}{|ll|} 
    \hline
        director: & pinkish \\
        matcher: & no pinks \\
        director: & not halloween orange \\
 \hline
 \end{tabular}
 \end{tabular}
 \caption{Alternate figure for Matthew}
\end{figure}

